Intelligent Reflecting Surfaces for Free Space Optical Communications

In this paper, we investigate the use of intelligent reflecting surfaces (IRSs) (i.e., smart mirrors) to relax the line-of-sight requirement of free space optical (FSO) systems. We characterize the impact of the physical parameters of the IRS, such as its size, position, and orientation, on the quality of the end-to-end FSO channel. In addition, we develop a statistical channel model for the geometric and the misalignment losses which accounts for the random movements of the IRS, transmitter, and receiver due to building sway. This model can be used for performance analysis of IRS-based FSO systems. Our analytical results shows that depending on the angle between the beam direction and the IRS plane, building sway for the IRS has either a smaller or larger impact on the quality of the end-to-end FSO channel than building sway for the transmitter and receiver. Furthermore, our simulation results validate the accuracy of the developed channel model and offer insight for system design.

==> Fig/Conditional/CondGML.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA Prop. Approx. (15)}%
\psfrag{019}[cl][cl]{\matlabtextA Exact (11), $a_r=100$~cm}%
\psfrag{020}[cl][cl]{\matlabtextA Exact (11), $a_r=50$~cm}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{13}{13}\selectfont\strut}%
\psfrag{022}[tc][tc]{\matlabtextB Misalignment [cm]}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextC $h_g$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextD $\matlabfragNegXTick 80$}%
\psfrag{002}[ct][ct]{\matlabtextD $\matlabfragNegXTick 60$}%
\psfrag{003}[ct][ct]{\matlabtextD $\matlabfragNegXTick 40$}%
\psfrag{004}[ct][ct]{\matlabtextD $\matlabfragNegXTick 20$}%
\psfrag{005}[ct][ct]{\matlabtextD $0$}%
\psfrag{006}[ct][ct]{\matlabtextD $20$}%
\psfrag{007}[ct][ct]{\matlabtextD $40$}%
\psfrag{008}[ct][ct]{\matlabtextD $60$}%
\psfrag{009}[ct][ct]{\matlabtextD $80$}%
\psfrag{010}[ct][ct]{\matlabtextD $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextD $10^{-6}$}%
\psfrag{012}[rc][rc]{\matlabtextD $10^{-5}$}%
\psfrag{013}[rc][rc]{\matlabtextD $10^{-4}$}%
\psfrag{014}[rc][rc]{\matlabtextD $10^{-3}$}%
\psfrag{015}[rc][rc]{\matlabtextD $10^{-2}$}%
\psfrag{016}[rc][rc]{\matlabtextD $10^{-1}$}%
\psfrag{017}[rc][rc]{\matlabtextD $10^{0}$}%
%
%% </ytick>

==> Fig/PDF/PDF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA $(\sigma_s,\sigma_r,\sigma_p)=(5,10,5)$~cm}%
\psfrag{008}[cl][cl]{\matlabtextA $(\sigma_s,\sigma_r,\sigma_p)=(5,5,10)$~cm}%
\psfrag{009}[cl][cl]{\matlabtextA $(\sigma_s,\sigma_r,\sigma_p)=(5,5,5)$~cm}%
\psfrag{010}[cl][cl]{\matlabtextA Prop. Model (16) and (20)}%
\psfrag{011}[cl][cl]{\matlabtextA Histogram (11) and (17)}%
\psfrag{012}[cl][cl]{\matlabtextA $A_0$}%
\psfrag{013}[cl][cl]{\matlabtextA 3D}%
\psfrag{014}[cl][cl]{\matlabtextA 2D}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{13}{13}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB PDF}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextC $h_g$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $10^{-3}$}%
\psfrag{001}[ct][ct]{\matlabtextD $10^{-2}$}%
\psfrag{002}[ct][ct]{\matlabtextD $10^{-1}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextD $10^{-2}$}%
\psfrag{004}[rc][rc]{\matlabtextD $10^{-1}$}%
\psfrag{005}[rc][rc]{\matlabtextD $10^{0}$}%
\psfrag{006}[rc][rc]{\matlabtextD $10^{1}$}%
%
%% </ytick>
